LearnAct: Few-Shot Mobile GUI Agent with a Unified Demonstration Benchmark

Mobile GUI agents show promise in automating tasks but face generalization challenges in diverse real-world scenarios. Traditional approaches using pre-training or fine-tuning with massive datasets struggle with the diversity of mobile applications and user-specific tasks. We propose enhancing mobile GUI agent capabilities through human demonstrations, focusing on improving performance in unseen scenarios rather than pursuing universal generalization through larger datasets. To realize this paradigm, we introduce LearnGUI, the first comprehensive dataset specifically designed for studying demonstration-based learning in mobile GUI agents, comprising 2,252 offline tasks and 101 online tasks with high-quality human demonstrations. We further develop LearnAct, a sophisticated multi-agent framework that automatically extracts knowledge from demonstrations to enhance task completion. This framework integrates three specialized agents: DemoParser for knowledge extraction, KnowSeeker for relevant knowledge retrieval, and ActExecutor for demonstration-enhanced task execution. Our experimental results show significant performance gains in both offline and online evaluations. In offline assessments, a single demonstration improves model performance, increasing Gemini-1.5-Pro's accuracy from 19.3% to 51.7%. In online evaluations, our framework enhances UI-TARS-7B-SFT's task success rate from 18.1% to 32.8%. LearnAct framework and LearnGUI benchmark establish demonstration-based learning as a promising direction for more adaptable, personalized, and deployable mobile GUI agents.

==> tables/tab-k-shot-results.tex <==
\begin{table*}[t]
	\definecolor{ForestGreen}{RGB}{34,139,34}
	\definecolor{NegativeRed}{RGB}{220,20,60}
	\newcommand{\hgreen}[1]{\textcolor{ForestGreen}{#1}}
	\caption{
		\textbf{Performance comparison of different models under various k-shot settings (accuracy \%).}
	\textmd{Four metrics shown for each model (Gemini-Pro-1.5, Qwen2-VL-7B, UI-TARS-7B-SFT) at 0-shot baseline vs. 1/2/3-shot performance: Step Type Accuracy, Step Complete Accuracy, Episode Type Accuracy, and Episode Complete Accuracy, with $\Delta$ indicating absolute improvement.}
	}
    \vspace{-2mm}
    \label{tab:k_shot_results}
    \begin{center}
    \setlength{\tabcolsep}{5.5pt}
    \renewcommand{\arraystretch}{1.1}
    {
    \begin{tabular}{l@{\hspace{4pt}}c@{\hspace{7pt}}|@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Examples}} & \textbf{Step Type} & \textbf{Step Complete} & \textbf{Episode Type} & \textbf{Episode Complete} \\
    & & \textbf{Accuracy} & \textbf{Accuracy} & \textbf{Accuracy} & \textbf{Accuracy} \\
    \midrule
    \multirow{6}{*}{Gemini-Pro-1.5} 
    & 0-shot & 68.2 & 19.6 & 0 & 0 \\
    & 1-shot & 81.6 & 50.4 & 16.7 & 0.9 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+13.4} & \cellcolor[HTML]{DAEFF9}\hgreen{+30.8} & \cellcolor[HTML]{DAEFF9}\hgreen{+16.7} & \cellcolor[HTML]{DAEFF9}\hgreen{+0.9} \\
    \cmidrule{2-6}
    & 0-shot & 68.7 & 19.4 & 0 & 0 \\
    & 2-shot & 81.7 & 54.7 & 12.8 & 2.4 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+13.0} & \cellcolor[HTML]{DAEFF9}\hgreen{+35.3} & \cellcolor[HTML]{DAEFF9}\hgreen{+12.8} & \cellcolor[HTML]{DAEFF9}\hgreen{+2.4} \\
    \cmidrule{2-6}
    & 0-shot & 68.8 & 19.3 & 0 & 0 \\
    & 3-shot & 83.0 & 57.7 & 17.1 & 3.2 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+14.2} & \cellcolor[HTML]{DAEFF9}\hgreen{+38.4} & \cellcolor[HTML]{DAEFF9}\hgreen{+17.1} & \cellcolor[HTML]{DAEFF9}\hgreen{+3.2} \\
    \midrule
    \multirow{9}{*}{Qwen2-VL-7B} 
    & 0-shot & 86.8 & 70.8 & 20.3 & 2.1 \\
    & 1-shot & 90.1 & 76.0 & 30.0 & 6.1 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+3.3} & \cellcolor[HTML]{DAEFF9}\hgreen{+5.2} & \cellcolor[HTML]{DAEFF9}\hgreen{+9.7} & \cellcolor[HTML]{DAEFF9}\hgreen{+4.0} \\
    \cmidrule{2-6}
    & 0-shot & 87.0 & 71.0 & 20.4 & 1.7 \\
    & 2-shot & 90.7 & 77.5 & 32.9 & 9.0 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+3.7} & \cellcolor[HTML]{DAEFF9}\hgreen{+6.5} & \cellcolor[HTML]{DAEFF9}\hgreen{+12.5} & \cellcolor[HTML]{DAEFF9}\hgreen{+7.3} \\
    \cmidrule{2-6}
    & 0-shot & 87.5 & 71.8 & 21.1 & 1.2 \\
    & 3-shot & 91.4 & 79.4 & 35.1 & 8.8 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+3.9} & \cellcolor[HTML]{DAEFF9}\hgreen{+7.6} & \cellcolor[HTML]{DAEFF9}\hgreen{+14.0} & \cellcolor[HTML]{DAEFF9}\hgreen{+7.6} \\
    \midrule
    \multirow{9}{*}{UI-TARS-7B-SFT} 
    & 0-shot & 91.1 & 77.1 & 35.5 & 8.2\\
    & 1-shot & 92.0 & 81.9 & 44.6 & 13.9  \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+0.9} & \cellcolor[HTML]{DAEFF9}\hgreen{+4.8} & \cellcolor[HTML]{DAEFF9}\hgreen{+9.1} & \cellcolor[HTML]{DAEFF9}\hgreen{+5.7} \\
    \cmidrule{2-6}
    & 0-shot & 91.4 & 77.2 & 36.0 & 8.7 \\
    & 2-shot & 91.5 & 81.1 & 38.1 & 11.8 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+0.1} & \cellcolor[HTML]{DAEFF9}\hgreen{+3.9} & \cellcolor[HTML]{DAEFF9}\hgreen{+2.1} & \cellcolor[HTML]{DAEFF9}\hgreen{+3.1} \\
    \cmidrule{2-6}
    & 0-shot & 91.7 & 77.5 & 37.1 & 8.8 \\
    & 3-shot & 91.9 & 82.1 & 40.6 & 13.2 \\
    & \cellcolor[HTML]{DAEFF9}$\Delta$ & \cellcolor[HTML]{DAEFF9}\hgreen{+0.2} & \cellcolor[HTML]{DAEFF9}\hgreen{+4.6} & \cellcolor[HTML]{DAEFF9}\hgreen{+3.5} & \cellcolor[HTML]{DAEFF9}\hgreen{+4.4} \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table*} 
